SWE-InfraBench: Evaluating Language Models on Cloud Infrastructure Code

Building infrastructure-as-code (IaC) in cloud computing is a critical task, underpinning the reliability, scalability, and security of modern software systems. Despite the remarkable progress of large language models (LLMs) in software engineering -- demonstrated across many dedicated benchmarks -- their capabilities in developing IaC remain underexplored. Unlike existing IaC benchmarks that predominantly center on declarative paradigms such as Terraform and involve generating entire codebases from scratch, our benchmark reflects the incremental code edits common in enterprise development with imperative tools like the AWS CDK. We present SWE-InfraBench, a diverse evaluation dataset sourced from dozens of real-world IaC codebases that challenge LLMs to perform realistic code modifications in AWS CDK repositories. Each example requires models to implement changes to existing codebases based on natural language instructions, with success determined by passing provided test cases. These tasks demand sophisticated reasoning about cloud resource dependencies and implementation patterns beyond conventional code generation challenges. Our evaluation results reveal significant limitations in current LLMs showing that even state-of-the-art systems struggle with many tasks -- the best model, Sonnet 3.7, succeeds in only 34\% of cases, while specialized reasoning models like DeepSeek R1 achieve just 24% success. The SWE-InfraBench dataset is available at: https://www.kaggle.com/datasets/64e59070fd51c0278560b01eb5dc4f3c447d5268cdabe5a350d2969e4413fea5

==> appx/benchmark.tex <==
\section*{Appendix}
\label{appx:intro}
In the appendix, we provide more thorough details regarding the dataset construction process, evaluation pipeline, and characterization of the \benchmark{} benchmark.

\section{Benchmark Details}
\label{appx:benchmark}

This section complements Section~\ref{sec:benchmark} with a more technical and fine-grained summary of the data collection, execution-based validation, and evaluation procedures, along with a fuller characterization of the task instances.

\subsection{High Level Overview}

\textbf{Pull request scraping.} From a list of the top $\num{5000}$ most downloaded PyPI libraries during August 2023\footnote{\href{https://hugovk.github.io/top-pypi-packages/}{https://hugovk.github.io/top-pypi-packages/}}, we select the top $100$ packages, identify each library's corresponding open-source GitHub repository, verify which packages have licenses allowing for free software use, and collect all PRs for these repositories via the GitHub developer API.
We elect to source problems from well-trafficked repositories because widespread use usually suggests that the repository has extensive documentation, structured open-source development guidelines, and working, well-formatted code.

\textbf{Task instance construction.} We construct candidate task instances from PRs that satisfy three conditions.
First, the PR's status must be \textit{Merged}.
A \textit{Merged} status indicates that the PR's associated code changes were accepted and incorporated into its parent repository. 
Second, the PR resolves one or more \textit{issues} in its repository.
An issue is defined according to its canonical usage in GitHub as a digital ticket for tracking bugs, enhancements, or any general development goals for a software project.
We scan a PR's title, body, and commit messages for linked issues (i.e. ``fixes \#$24$'').
Third, the PR must introduce one or more new tests.
A new test is counted when a PR's code changes edits a file path containing a testing-related keyword (e.g. ``test", ``testing").

A PR that satisfies these criteria is then converted into a candidate task instance such as the example in Figure~\ref{fig:example}.
The codebase $C$ is identified by the repository's owner/name moniker and the pull request's base commit.
Recovering the actual codebase from this information is straightforward.
We create mirrors of the original GitHub repositories, where each mirror is uniquely identified as \texttt{owner\_\_name}.
Cloning a repository's corresponding mirror and checking out the base commit yields $C$ in its pre-PR state.
The problem statement $P$ is an aggregate of all related issues' titles and descriptions along with any subsequent comments written before the timestamp of the PR's initial commit to avoid leakage of solution details.
A PR's code changes are separated into a test patch and a gold patch $\delta$. $T$ consists of all tests from files edited in the test patch.
As shown in Figure~\ref{fig:example}, both $T$ and $\delta$ are stored as \texttt{patch} files.
Further details about parsing PR and semantic data is in Appendix~\ref{appx:benchmark:construction}.

\input{figures/example-task}

\textbf{Execution-based validation.} We verify the usability of a task instance via execution. 
For each candidate, we first define a virtual environment to serve as an execution context, then install $C$ before applying any patches, and finally run $T$ once before and once after the solution $\delta$ is applied.
A candidate is removed from consideration for the final dataset if any step in the verification process fails.
In addition, to ensure that a solution $\delta$ is non-trivial, we compare the pre-solution and post-solution validation logs to check for whether there are one or more tests in $T$ where the status changes from \textit{fail} to \textit{pass}.
Lastly, we exclude task instances with tests that invoke newly created functions or classes first introduced in the solution $\delta$.
Since naming such constructs is typically an arbitrary process and usually not explicitly specified in the problem statement, resolving tests such as these may be an impossible task even for human developers.
Information about execution contexts, codebase installation, determining test statuses from logs, and more are in Appendix~\ref{appx:benchmark:exec-validation}.

\textbf{Continuous Updates.} \benchmark{}'s collection process is easily extensible to any open source code repositories, allowing for easy and low-maintenance extension to new programming languages and code domains.
This design also provides \benchmark{} with temporal robustness; as new language models trained on more recent source code are released over time, \benchmark{} can simply be updated to produce new task instances based on PRs created after any LM's training date.


\subsection{Construction Process}
\label{appx:benchmark:construction}
We discuss additional details regarding the conversion of a pull request object into a candidate task instance.
At a high level, the main goal of this conversion is to acquire relevant information for putting together the codebase $C$, problem statement $P$, unit tests $T$, and solution $\delta$ components introduced in Section~\ref{sec:benchmark}.
To this end, a \benchmark{} task instance consists of the following fields, presented in the following Table~\ref{table:task-instance-fields}.
Collectively, the fields correspond to the four task instance modules.

\input{tables/appx/task-instance-fields}

\textbf{Problem Statement.} The problem statement $P$ for each task instance is readily available as the \texttt{problem\_statement} field.
The problem statement is an aggregate of all issues' first comments along with any comments attached to those issues that were created before the creation date of the PR's initial commit.
We crawl for issues from PR's title, body, and commit messages. After concatenating these components' text data, we first remove any Markdown-style comments, then look through the remaining text for references to issue numbers (a pound \# sign followed by a number) and check whether the word preceding the issue number reference is included in a set of keywords suggesting that the issue was resolved by the PR (e.g. ``closes'', ``fixes'', ``resolves'').
The found issues are recorded in the \texttt{issue\_numbers} field, then separate web requests are made to retrieve each issue's data.
To form the \texttt{problem\_statement}, each issue's title and body are added together and then concatenated with the next issue's if there are multiple.
It is also during this step that the \texttt{hints\_text} field is created and collected from the PR's comment section, where text from comments created before the PR's initial commit.
The intuition for this collection methodology is that such PR comments would likely contain natural language and pseudo-code suggestions to the original human task worker regarding how to complete the problem at hand. 
The experiments presented in this work do not make use of \texttt{hints\_text}, but we believe this information may be interesting for future investigations.

\textbf{Codebase.} The codebase $C$ content is \textit{not} stored in plaintext for every task instance. 
Rather, the task instance contains a reference to the relevant codebase via the \texttt{repo} and \texttt{base\_commit} field.
Both fields are available in the original PR's data. To make retrieval of the codebase $C$ from these two elements reproducible and reliable, we create mirrors\footnote{\href{https://docs.github.com/en/repositories/creating-and-managing-repositories/duplicating-a-repository}{Documentation} for creating a mirror repository using GitHub} of the original repository.
Mirrors for the repository constituting both the evaluation and fine tuning data are collected and open-sourced under the \benchmark{} GitHub organization.
Because an original repository's code may be subject to changes in its commit and edit history outside of the authors' control, we choose to create a mirror repository to ensure that later modifications to the codebase do not potentially render a task instance unusable due to a corruption or removal of the associated \texttt{base\_commit}.
Additionally, we create a mirror instead of cloning and storing the latest version of a repository. This is because a mirror retains the original commit hashes, history, branches, and tags, serving as a faithful and complete history of the technical details of the original repository.
A mirror does not retain stars, watchers, issues, or pull requests from the original repository.

We create a mirror from a repository after and within the same day when task instances were collected.
The mirror retains the original repository's ``\texttt{owner}/\texttt{name}'' moniker, except that the ``/'' character is converted to a ``\_\_'' to confirm to GitHub naming conventions.
Given this infrastructure, retrieving a task instance's codebase is straightforward.
First, the correct mirror can be cloned from the \benchmark{} organization using \texttt{repo}.
Next, within the local copy of the mirror, checking out the \texttt{base\_commit} will reset the repository to codebase $C$.
To proceed to another task instance from the same repository, \texttt{git} version control is used to automatically remove any modifications associated with the current task instance before checking out the next task instance's base commit.

\textbf{Solution, Test Patches.}
The solution $\delta$ and tests $T$ are derived from the file changes data, or \texttt{diff}, of a PR.
As mentioned in Section~\ref{sec:benchmark:construction}, the original \texttt{diff} along with solution $\delta$ and tests $T$ are represented as a \texttt{.patch} file, a format for efficiently specifying transformations to line-based text files.
Generally speaking, a \texttt{.patch} is structured as a list of blocks, where each block consists of a header and one or more hunks that collectively correspond to changes to a single file.
The header contains metadata specifying a file path and line numbers, while the actual modifications to the target file are encoded as multiple lines prefixed by ``+'' and ``-'' to indicate additions and removals.
To create the tests $T$, we first identifying every unique block within the patch, then pick out and conglomerate blocks with file paths that contain testing-related keywords (e.g. ``tests'', ``testing'').
The remaining blocks are merged to form the solution $\delta$.
We validate the robustness of the script written to parse correctly $T$ and $\delta$ by applying both patches to the corresponding codebase $C$ and running the tests; we then check that the results reproduce the behavior of the base PR's \texttt{diff} data.
The solution $\delta$ is saved as the \texttt{patch} field while the tests $T$ are saved as the \texttt{test\_patch} field.

\textbf{Remaining Fields.} The \texttt{created\_at} field is a timestamp that specifies when the base PR was created.
We retain the \texttt{created\_at} field from the original data and use this field to perform temporal analysis of model performance.
The \texttt{version} field is a string that corresponds to the release version, with respect to the \texttt{repo}, during which the PR was released.
Depending on availability and the amount of effort required for each method, we create the \texttt{version} field by retrieving the information directly from the source code, building the repository locally and invoking code to display the version to standard output, or comparing the \texttt{created\_at} field with a timeline of release versions from a repository's webpage.
We create executable contexts for every \texttt{version} of a repository, as discussed in greater detail in \S~\ref{appx:benchmark:exec-validation}.

\subsection{Execution-Based Validation}
\label{appx:benchmark:exec-validation}

After filtering through all the PRs from a repository and converting those that satisfy the aforementioned criteria into candidate task instances, the next step is to validate the usability of each task instance via execution.
This procedure is broken down into three steps.
First, we create executable contexts for each release version of a repository.
Next, we check whether the solution $\delta$ and tests $T$ can be applied, installed, and run successfully on top of codebase $C$.
Finally, we examine each task instance's execution log to verify a specific set of behaviors to ensure that the task is usable and fair for model evaluation.

\textbf{Executable Contexts.} We choose to create executable contexts per release version after experimenting with various degrees of granularity with regards to what definition level to define virtual environments for. 
Defining task instance-specific contexts is most conducive to ensuring end-to-end installation success, but comes at the cost of laborious manual handcrafting.
On the other hand, a repository-specific context based on the latest version of a repository is typically too coarse of a definition that is not compatible with older versions' requirements.
We find that release versions are a good proxy for capturing the dependency requirements across a subset of task instances, striking a manageable balance between installation success and manual effort.
We manually create each executable context by examining the codebase of the \textit{latest} task instance for each version.
Based on the source code and documentation typically found in the repository's \texttt{README} and \texttt{CONTRIBUTING} guides, we find out the Python version, necessary dependencies, and installation command.

\textbf{Validation Engine.}
The purpose of the validation engine is to verify candidate task instances. Specifically, this step checks first, that the solution $\delta$ and tests $T$ can be applied to codebase $C$, and second, that the codebase can be properly installed and run within the corresponding virtual environment.
To do this, we perform validation repository-by-repository, where for each repository's set of task instances, we perform the following procedure:

\begin{enumerate}
    \item Create executable contexts as \texttt{conda} envs. based on latest task instance per \texttt{version}.
    \item Group task instances by \texttt{version}.
    \item Iterate across each task instances group, where for each task instance, we perform the following within the corresponding \texttt{conda} env.
    \begin{enumerate}
        \item Remove any file changes and checkout the task instance's \texttt{base\_commit}. This sets the repository to codebase $C$.
        \item Run the installation command to instantiate codebase $C$.
        \item Apply the test patch $T$ to codebase $C$.
        \item Run the testing script, determined from test patch $T$, to generate test result logs $log_{pre}$.
        \item Apply the solution $\delta$ patch to the codebase $C$ with tests $T$.
        \item Run the testing script from part (d) again to generate test result logs $log_{post}$.
    \end{enumerate}
\end{enumerate}

The testing command consists of the testing framework used by the repository (e.g. \texttt{pytest}, \texttt{tox}) with paths specified in $T$ appended.
The testing command would run any and all tests that are specified within the contents of each file path.
If any of the steps $(a)$ through $(f)$ fails, the candidate task instance is discarded from consideration.
With moderate variation across repositories, we observe that this step generally removes half of the candidate task instances.

\input{tables/appx/repo-conversion-stats}

\textbf{Examining Validation Logs.}
Last but not least, we check the logs $log_{pre}$ and $log_{post}$ created by the validation engine for specific properties.
First, to guard against arbitrary naming choices, we check $log_{pre}$ for \texttt{ImportError} and \texttt{AttributeError} occurrences, which are potentially indicative of dependency naming related errors that would trivial and near-impossible to address correctly.
To this end, we remove all task instances with such errors in their $log_{pre}$ from consideration.
Next, we compare the test results to check that the task instance is non-trivial, indicated by at least one or more tests having a \texttt{fail} status before the solution $\delta$ is applied, then a \texttt{pass} status after.
To check this, we first define several repository-specific parsers to convert $log_{pre}$ and $log_{post}$ into mappings of test $t_i \in T$ to a status $s \in$ [\textit{fail},\textit{pass}].
Given these two data structures, we then check that there exists at least one $t_i$ where $s$ changes from \textit{fail} to \textit{pass}.
If no such tests are found, the task instance is removed from consideration.

If a task instance fulfills these two criteria, then it is included in the evaluation dataset.
Table~\ref{table:repo-conversion-stats} displays a summary of how many task instances were removed from consideration across the construction process and execution based validation steps.
We save all finalized task instances to a single \texttt{.json} file that is open sourced and available for download.

Alongside the task instances, we also create a corresponding folder containing the ground truth test results.
For each task instance, from their respective $log_{pre}$ and $log_{post}$ test-to-status mappings, we create a test results data structure where the keys are \texttt{FAIL\_TO\_FAIL}, \texttt{FAIL\_TO\_PASS}, \texttt{PASS\_TO\_FAIL}, and \texttt{PASS\_TO\_PASS}, and the values are lists of tests.
By ``caching" these results, we remove the need to re-run the solution $\delta$ at evaluation time (although re-running is an available option).
We use this data structure to verify task completion, as discussed in Section~\ref{appx:benchmark:eval-procedure}.

\subsection{Evaluation Procedure}
\label{appx:benchmark:eval-procedure}

\input{figures/evaluation-pipeline}

We provide a visualization of the evaluation procedure in Figure~\ref{fig:eval-pipeline}.
The evaluation procedure scores the model's $\hat{\delta}$ \texttt{.patch} generation with respect to the behavior of the solution $\delta$.
At a finer-grained level, the evaluation procedure can be broken down into four separate steps, highlighted by the numbered steps in Figure~\ref{fig:eval-pipeline}.
First, the codebase and problem statement are visible and given to the LM; the LM then generates a \texttt{.patch} prediction $\hat{\delta}$.
In the evaluation step, the following steps are performed per prediction on the target task instance:

\begin{enumerate}
    \item Remove any file changes and checkout the task instance’s base commit. This sets the repository to codebase $C$.
    \item Activate the executable context corresponding to the task instance's \texttt{version}.
    \item Run installation command to instantiate codebase $C$.
    \item Apply test patch $T$ to codebase $C$.
    \item Apply prediction patch $\hat{\delta}$ to codebase $C$ with tests $T$.
    \item If the previous step fails, we attempt to fix prediction patch $\hat{\delta}$ automatically and reapply it.
    \item Run the testing script, determined from test patch $T$, to generate test result logs $log_{\hat{\delta}}$.
\end{enumerate}

Steps 1 through 4 reliably do not fail due to verification during the task instance validation process. If applying the prediction patch (Step 5) fails, we attempt to repair the prediction patch file by removing unnecessary context lines and recalculating the header values (Step 6). If the remaining patch fails again or running the test command (Step 7) fails, then the prediction is automatically given a score of $0$. Assuming these steps succeed, the output log $log_{\hat{\delta}}$ can then be converted to a test-to-status mapping, identical in structure to the  via the appropriate, repository-specific parser introduced in \S~\ref{appx:benchmark:exec-validation}.

\textbf{Evaluation Metrics Calculation.}
To determine task completion, we compare the test-to-status mapping parsed from $log_{\hat{\delta}}$ with the list of tests corresponding to the \texttt{FAIL\_TO\_PASS} and \texttt{PASS\_TO\_PASS} keys from the ground truth test results data structure.
Determining task completion is straightforward; we check that all \texttt{FAIL\_TO\_PASS} and \texttt{PASS\_TO\_PASS} tests are found and have a \textit{pass} status in the evaluation test-to-status mapping.
If a test is missing or has a non-\textit{pass} status, it is considered a \textit{fail} status. As defined and used in the main paper, a task is considered solved if all tests across \texttt{FAIL\_TO\_PASS} and \texttt{PASS\_TO\_PASS} pass.

\subsection{Evaluation Test Set Characterization}
\label{appx:benchmark:repo-stats}

\input{tables/appx/repo-dataset-stats}

We include an expanded form of Table~\ref{table:dataset-stats} that includes repository specific statistics in Table~\ref{table:repo-dataset-stats}.
Table ~\ref{table:repo-summaries} presents a brief description of each repository extracted from the repository's documentation along with the repository's associated open source license.
The associated licenses all permit non-commercial usage of the original library source code as long as the permissions in the original licenses are upheld and retained.
In addition to the original statistics presented in Table~\ref{table:dataset-stats}, we introduce three new values.
The $\delta$ \# Lines Added and $\delta$ \# Lines Removed together sum up to $\delta$ Lines Edited. ``Added" refers to the number of new lines that are introduced, while ``Removed" are pre-existing lines taken out by the solution.
The $\vert T \vert$ (Pass to Pass) statistic refers to the number of tests that were passing before the solution $\delta$ was applied during the validation pipeline.
Unlike \textit{fail} to \textit{pass} tests that are intended to characterize the problem statement $P$ and determine if a revision addresses the issue, \textit{pass} to \textit{pass} tests are included to ensure that the revision does not break or violate any existing expected behavior.
These tests are extracted during the validation log examination phase as discussed in \S~\ref{appx:benchmark:exec-validation}.
We note that \textit{fail} to \textit{fail} tests and \textit{pass} to \textit{fail} tests are not considered during evaluation, and those statistics are not reflected in the above table.

\input{tables/appx/repo-summaries}

\textbf{Task Instance Issue Categories.} To provide a better sense of the types of problems that \benchmark{} task instances include, we perform simple analyses on the issues, identified by the \texttt{issue\_numbers} field, for each task instance.
Per issue, we inspect metadata, specifically tags, to characterize the type of contribution put forth by the PR.
Table~\ref{table:issue-tags} groups and shows several examples of the $\num{2289}$ tags we found across all issues.
While the absolute majority of issues are associated with bug fixes, \benchmark{}'s task instances are associated with a diverse set of code changes with purposes beyond debugging and error correction.

\input{tables/appx/issue-tags}

\textbf{Attribute Distributions.} In Figure~\ref{table:dataset-stats-cdfs}, we present plots of the cumulative distribution function for attributes introduced in Table~\ref{table:dataset-stats}.
From these plots, we see that the median \benchmark{} task instance has a problem description of $140$ words, and will take place within a codebase containing just shy of $1900$ files and $400$K lines.
The corresponding reference solution $\delta$ will usually edit a single function within a file, changing $\sim$$15$ lines, and has a single \textit{fail} to \textit{pass} test to verify the correctness of the change along with $51$ \textit{pass} to \textit{pass} tests to check whether existing behavior is preserved.

\input{figures/dataset-stats-cdfs}

\textbf{Patch Fix Rate.} We present Table~\ref{table:patch-fix-rates}, which presents summary statistics of how many task instances each model generated patches for (out of 2294), how many of these patches applied successfully, and how many of the successfully applied patches required undergoing the patch fixing procedure introduced in Appendix~\ref{appx:benchmark:eval-procedure}.
We find that fixed patches tend to make up a smaller percentage of the \swellama{} patches that successfully applied, suggesting that \swellama{}'s fine tuning procedure has a positive effect on generating well-formatted patches.
For closed source models, fewer patches apply successfully, and of the ones that do, a greater percentage require the post-generation fix, suggesting that models still struggle with patch generation and structured outputs in general.

\input{tables/appx/patch-fix-rates}

\subsection{Development Set Characterization}

In addition to the evaluation test set, we also provide a development set for evaluating models and tuning hyperparameters before running on the final test set.
Following the style of tables and graphs from before, we present similar statistics to characterize the $225$ development task instances (slightly more than $10$\% of the main evaluation set) collected from $6$ open source repositories with licenses permitting such usage.
The development set was collected following the exact same set of methodologies and filters as the main evaluation set.
In addition to the pre-existing steps, we also filter the development set to keep task instances that were created after January $1$, $2019$.
Similar to Table~\ref{table:repo-summaries}, in Table~\ref{table:dev-repo-summaries}, we briefly summarize the purpose and licenses of the $6$ selected repositories.

\input{tables/appx/dev-repo-summaries}

Following Table~\ref{table:issue-tags}, we also list the tags associated with the the development set tasks in Table~\ref{table:dev-issue-tags}, again showcasing the diversity and coverage of task types beyond fixing bugs.
Compared to the main evaluation tasks, we can also see tags (e.g., ``Crash :collision:", ``io") that refer to issues presenting problems which are unique to the repositories in the development set.

\input{tables/appx/dev-issue-tags}

Following Table~\ref{table:dataset-stats}, we present the same set of repository-specific average statistics for the $6$ repositories in the development set in Table~\ref{table:dev-repo-dataset-stats}.
Across the entire development set, each task instance has $19.9$ average / $2$ median F2P tests.
There are $171.3$ average / $79.0$ median P2P tests, and $191.2$ average / $101.0$ median tests in total per task instance.

\input{tables/appx/dev-repo-dataset-stats}

\subsection{SWE-bench Lite Characterization}
\label{appx:benchmark:lite}
SWE-bench Lite is a canonical subset for more efficient evaluation of languag models on the SWE-bench task.
SWE-bench is 


==> appx/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? \answerYes{} The claims in the abstract and introduction are accurately aligned with the actual scope of the paper, which introduces a novel infrastructure-as-code benchmark.
    % \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: The claims in the abstract and introduction are accurately aligned with the actual scope of the paper, which introduces a novel infrastructure-as-code benchmark.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
    %     \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
    %     \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
    %     \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    % \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors? \answerYes{} The Conclusion section discusses some limitations and possible future extensions of the introduced benchmark and empirical experiments conducted in the paper.
    % \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: The Conclusion section discusses some limitations and possible future extensions of the introduced benchmark and empricial experiments conducted in the paper.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
    %     \item The authors are encouraged to create a separate "Limitations" section in their paper.
    %     \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
    %     \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
    %     \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
    %     \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
    %     \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
    %     \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    % \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof? \answerNA{} The paper does not include any theoretical results.
    % \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: The paper does not include any theoretical results.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include theoretical results. 
    %     \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
    %     \item All assumptions should be clearly stated or referenced in the statement of any theorems.
    %     \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
    %     \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
    %     \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    % \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?  \answerYes{} The paper provides a description of the benchmark construction as well as empirical experiments conducted on it. We publish the complete dataset, disclose the links and licenses of the donor repositories, and the code implementing the benchmark construction pipeline and the evaluation experiments for different models and approaches tested in the paper. This allows reproducing our results, or extending the analysis by evaluating techniques not considered in this paper.
    % \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: The paper provides a description of the benchmark construction as well as empirical experiments conducted on it. We publish the complete dataset with 100 tasks, disclose the links and licenses of the donor repositories, and the code implementing the benchmark construction pipeline and the evaluation experiments for different models and approaches tested in the paper. This allows reproducing our results, or extending the analysis by evaluating techniques not considered in this paper.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
    %     \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
    %     \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
    %     \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
    %     \begin{enumerate}
    %         \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
    %         \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
    %         \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
    %         \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
    %     \end{enumerate}
    % \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material? \answerYes{} The paper provides access to the data and code, with instructions to reproduce the main experimental results and analyze the dataset entries.
    % \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: The paper provides access to the data and code, with instructions to reproduce the main experimental results and analyze the dataset entries. 
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that paper does not include experiments requiring code.
    %     \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
    %     \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
    %     \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
    %     \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
    %     \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
    %     \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
    %     \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    % \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results? \answerYes{} The paper provides the prompt templates, LLM inference parameters, and evaluation metrics definitions for the provided evaluation experiments.
    % \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: The paper provides the prompt templates, LLM inference parameters, and evaluation metrics definitions for the provided evaluation experiments.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
    %     \item The full details can be provided either with the code, in appendix, or as supplemental material.
    % \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments? \answerNo{} We do not perform statistical significant tests of the overall model performance due to high costs of repeated LLM calls. At the same time, we provide additional analysis, including error distribution analysis and investigate performance of selected LLMs in a setting with multiple independent generations, presented in the main paper and in the Appendix. This provides insights on the consistency of the observed results. 
    % \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: We do not perform statistical significant tests of the overall model performance due to high costs of repeated LLM calls. At the same time, we provide additional analysis, including error distribution analysis and investigate performance of selected LLMs in a setting with multiple independent generations, presented in the main paper and in the Appendix. This provides insights on the consistency of the observed results. 
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
    %     \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
    %     \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
    %     \item The assumptions made should be given (e.g., Normally distributed errors).
    %     \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
    %     \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
    %     \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
    %     \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    % \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments? \answerNo{} The paper focuses on benchmarking LLMs available via API calls by different model providers, which does not create any non-standard computer resources to reproduce the experiments.
    % \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: The paper focuses on benchmarking LLMs available via API calls by different model providers, which does not create any non-standard computer resources to reproduce the experiments.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
    %     \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
    %     \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    % \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}? \answerYes{} Justification: The research conforms with the NeurIPS Code of Ethics.
    % \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: The research conforms with the NeurIPS Code of Ethics.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
    %     \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
    %     \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    % \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed? \answerNA{} The benchmark targets low-level infrastructure code modifications without direct interaction with end users or social systems, and thus does not raise immediate concerns around fairness, privacy, or misuse.
    % \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: \justificationTODO{}
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that there is no societal impact of the work performed.
    %     \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
    %     \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
    %     \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
    %     \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
    %     \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    % \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)? \answerNA{} The paper poses no substantial risks of misuse.
    % \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: the paper poses no substantial risks of misuse.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper poses no such risks.
    %     \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
    %     \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
    %     \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    % \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected? \answerYes{} The paper provides a list of licenses for the donor repositories that were used to construct the benchmark. 
    % \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: the paper provides a list of licenses for the donor repositories that were used to construct the benchmark. 
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not use existing assets.
    %     \item The authors should cite the original paper that produced the code package or dataset.
    %     \item The authors should state which version of the asset is used and, if possible, include a URL.
    %     \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
    %     \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
    %     \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
    %     \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
    %     \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    % \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets? \answerYes{} The paper provides documentation of the introduced asset -- a new benchmark dataset for infrastructure-as-code generation.
    % \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: the paper provides documentation of the introduced asset -- new benchmark dataset for infrastructure-as-code generation.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not release new assets.
    %     \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
    %     \item The paper should discuss whether and how consent was obtained from people whose asset is used.
    %     \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    % \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? \answerNA{} The paper does not involve crowdsourcing nor research with human subjects.
    % \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
    %     \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
    %     \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    % \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained? \answerNA{} The paper does not involve crowdsourcing nor research with human subjects.
    % \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
    %     \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
    %     \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
    %     \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    % \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required. \answerYes{} As described in the paper, we use a semi-automated pipeline for generating dataset examples using LLMs. The process is documented in detail in Section 2, and prompt examples are provided in the Appendix.
    %this research? 
    % \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: as described in the paper, we use a semi-automated pipeline for generating dataset examples using LLMs. The process is documented in detail in Section 2, and prompt examples are provided in the Appendix.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
    %     \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    % \end{itemize}

\end{enumerate}

==> appx/experimental-details.tex <==
\section{Additional Experimental Details}
\label{appx:experiment-details}

\subsection{Retrieval Details}
\label{appx:retrieval}

\textbf{Sparse retrieval.}
During retrieval we make a slight augmentation to the documents by pre-pended files' contents with their file paths to better enable retrieval based on filenames that may be mentioned directly in the issue.

\textbf{Oracle retrieval.}
Oracle retrieval file paths are simply extracted directly from the reference solution's patch file excluding test files.

\subsection{Inference Settings}
Since generations are relatively expensive, we only generate a single patch file per instance. Following precedent in code generation for evaluation in Pass@$1$~\citep{chen2021evaluating,rozière2023code}, we simply use greedy decoding for all models.

\subsection{Prompt Template Example}
\label{appx:experimental-setup:prompt-template-example}
Models are prompted with the following general template with slight variations depending on the model used.
\begin{lstlisting}
You will be provided with a partial code base and an issue statement explaining a problem to resolve.
<issue>
{ISSUE TEXT}
</issue>

<code>
[start of README.md]
{README.md text}
[end of README.md]
[start of file_1.py]
{file_1.py text}
[end of file_1.py]
...
</code>

Here is an example of a patch file. It consists of changes to the code base. It specifies the file names, the line numbers of each change, and the removed and added lines. A single patch file can contain changes to multiple files.

<patch>
--- a/file.py
+++ b/file.py
@@ -1,27 +1,35 @@
 def euclidean(a, b):
-    while b:
-        a, b = b, a % b
-    return a
+    if b == 0:
+        return a
+    return euclidean(b, a % b)
 
 
 def bresenham(x0, y0, x1, y1):
     points = []
     dx = abs(x1 - x0)
     dy = abs(y1 - y0)
-    sx = 1 if x0 < x1 else -1
-    sy = 1 if y0 < y1 else -1
-    err = dx - dy
+    x, y = x0, y0
+    sx = -1 if x0 > x1 else 1
+    sy = -1 if y0 > y1 else 1
 
-    while True:
-        points.append((x0, y0))
-        if x0 == x1 and y0 == y1:
-            break
-        e2 = 2 * err
-        if e2 > -dy:
+    if dx > dy:
+        err = dx / 2.0
+        while x != x1:
+            points.append((x, y))
             err -= dy
-            x0 += sx
-        if e2 < dx:
-            err += dx
-            y0 += sy
+            if err < 0:
+                y += sy
+                err += dx
+            x += sx
+    else:
+        err = dy / 2.0
+        while y != y1:
+            points.append((x, y))
+            err -= dx
+            if err < 0:
+                x += sx
+                err += dy
+            y += sy
 
+    points.append((x, y))
     return points
</patch>

I need you to solve the provded issue by generating a single patch file that I can apply directly to this repository using git apply. Please respond with a single patch file in the format shown above.

Respond below:
\end{lstlisting}

Experiments using slightly more or fewer lines of instructions or examples seemed to not affect overall performance substantially, except for the findings of experiments stated in Section~\ref{sec:results}.


==> appx/miscellaneous.tex <==
\section{Societal Impact}
\label{appx:societal-impact}
As reasoning on code has emerged as a foundational skill underlying many LM's capability, a potential future of machine-automated software engineering raises many important questions and has important potential ramifications with regards to AI Safety~\citep{gros2023ai}.
It is important to address questions on how to ensure AI-generated code is faithful to human intents and what guardrails might be in place when human objectives are misinterpreted by code agents that then carry out the task.
To observe such problems in a controlled setting and manifest their solutions, we hope \benchmark{} might serve as a testbed for designing safe, robust measures 
towards aligned, verifiable, and safe AI-driven software engineering.

==> appx/quality-analysis.tex <==
\section{In-depth Analysis of \swellama{} Generations}
\label{appx:extra-results:quality-in-depth}

In this section, we provide five additional qualitative analyses of generations from both Claude 2 and \swellama{} generations (Oracle retrieval setting) following the style of Section~\ref{sec:results:quality-study}.

Claude 2 qualitative studies can be found in Tables~\ref{table:appx:quality-example6} and ~\ref{table:appx:quality-example7}.
Tables ~\ref{table:appx:quality-example8}, ~\ref{table:appx:quality-example9}, and ~\ref{table:appx:quality-example10} are task instances that Claude 2 did not address correctly.
\swellama{} qualitative studies are covered across Tables~\ref{table:appx:quality-example1}, ~\ref{table:appx:quality-example2}, ~\ref{table:appx:quality-example3}, ~\ref{table:appx:quality-example4}, ~\ref{table:appx:quality-example5}.
For Tables~\ref{table:appx:quality-example1}, ~\ref{table:appx:quality-example2}, and ~\ref{table:appx:quality-example3}, we present task instances solved correctly by \swellama{} 13b.
In Table~\ref{table:appx:quality-example4} and ~\ref{table:appx:quality-example5}, we present two task instances where \swellama{} 13b does not address the issue correctly, pointing out a subset of the reasoning and generation skills that models may not be adept at enough to accomplish the task at hand.

The observations we make across these sections corroborate with the points stated in the main paper, which is that models tend to struggle with multi-line and multi-file changes, are more adept when the required fix is relatively short, and need help with understanding the codebase in an efficient manner.

\input{tables/quality-analyses/example6}
\input{tables/quality-analyses/example7}
\input{tables/quality-analyses/example8}
\input{tables/quality-analyses/example9}
\input{tables/quality-analyses/example10}
\input{tables/quality-analyses/example1}
\input{tables/quality-analyses/example2}
\input{tables/quality-analyses/example3}
\input{tables/quality-analyses/example4}
\input{tables/quality-analyses/example5}

==> appx/results.tex <==
\section{Additional Results}
\label{appx:extra-results}

\subsection{Results with ``Oracle'' Retrieval}
\input{tables/appx/oracle-results}
Using the ``oracle'' retrieval method described in Section~\ref{sec:experimental-setup:input-formulation}, we show the general performance results in Table~\ref{table:main-results-oracle}. Naturally, providing only the files edited by the reference solution's pull request, model performance improves compared to the noisier BM25 retrieval setting.

\subsection{Evaluation Test Set}
\input{tables/appx/main-results-repo}
We include a repository-by-repository breakdown of model performance in Table~\ref{table:main-results-repo} that corresponds to Figure~\ref{fig:per-repo-oracle-fig} in the main paper. As discussed, in the main paper, performance differs heavily across repositories.

\subsection{GPT-4 Evaluation Subset Results}
In this section, we present the statistics shown in Table~\ref{table:main-results} for the $25$\% random subset that GPT-4 was tested in Table~\ref{table:main-results-20}.
As the selection of the subset is random, we find that the \% Resolved and \% Apply rates are consistent with the main results, and not significantly skewed towards being simpler or more difficult than the general evaluation set.

\input{tables/appx/main-results-20}

\subsection{Extended Temporal Analysis}

In this section, we present an extended temporal analysis of task instances solved by year that follows the analysis shown in Table~\ref{table:temporal-results} of the evaluation section in the main paper.
In Table~\ref{appx:temporal-results-extended}, we present the \% Resolved statistic across models under the ``Oracle" retrieval setting for $6$ different temporal partitions that group tasks by the years in which the issues were created.
It is evident from the table that there is no consistent correlation between model performance and year, supporting our conclusion that despite having potentially seen older versions of code within its pre-training datasets, understanding and implementing in fixes in \benchmark{} is a difficult task that requires understanding and cannot be accomplished feasibly or consistently via memoization of observed data.

\input{tables/appx/temporal-results-extended}

\subsection{F2P, P2P Rate Analysis}

In the main paper results, we present the ``\% Resolved" statistic that indicates how many task instances were \textit{completely} solved by the different models.
In this section, we provide more fine-grained insight into the gap of task instances where 1. The model's patch generation was applied successfully and 2. The task instance was not resolved.
Assuming a patch is applied successfully, we define $6$ cases in Table~\ref{table:six-outcome-cases} that fully capture the distribution of all possible outcomes based on the pass/fail results of F2P and P2P tests.
In addition to the ``Resolved" outcome that has been established, we introduce five new terms.
The ``Breaking Resolved" outcome refers to when the desired behavior of the issue has been accomplished (all F2P tests pass), but not all prior behavior is maintained (not all P2P tests pass).
``Partially Resolved" refers to when prior behavior of a codebase was maintained (all P2P tests pass); however, the desired behavior is not fully accomplished (not all F2P tests pass).
The ``Work in Progress" case is when the desired behavior is not fully accomplished (not all F2P tests pass) and the prior behavior of the codebase is not maintained (not all P2P tests pass).
A ``No-Op" is when a code change does not have any effect on the original codebase; prior behavior is maintained (all P2P tests pass) but the issue remains completely unresolved ($0$ F2P tests pass).
Finally, if the issue is unresolved ($0$ F2P tests pass) and prior working behavior is reverted (some P2P tests fail), the codebase is left in a worse state, which we define to be a ``Regression".

\input{tables/appx/six-outcome-cases}

In Table~\ref{table:six-outcome-stats}, we categorize patch generations that successfully applied according to these six cases.
We find that of non-``Resolved" issues, the majority of patch generations proposed by the model do not solve a single F2P test case from the corresponding task instance (``No-Op" and ``Regression").
Within the subset of these cases, the majority ($60\%$ to $70\%$) of cases are a No-Op, while the model breaks existing behavior for the remainder of these situations.

\input{tables/appx/six-outcome-stats}

Generally, the cases where model generations pass some, but not all tests (``Breaking Resolved", ``Partially Resolved", ``Work in Progress") cumulatively represent a smaller subset of problems relative to the other three categories.
From manual inspection of several of these cases, it is clear that the model demonstrates some understanding of the task requirements.
However, due to the baseline methods' limited view of the codebase that does not include information such as inter-file dependencies and functions' relationships, for many of these task instances often fail because a change that correctly resolves the immediate issue does not account for other modules that use and are affected by the changed entity.
We include several case studies that directly highlight these shortcomings in Section~\ref{appx:extra-results:quality-in-depth}
Overall, these results highlight not just the difficulty of \benchmark{}, but also point to the potential value of providing feedback via an execution environment that would allow models to run fixes against existing tests, then decide whether to continue editing or submit the patch for review.

\subsection{Patch Generation Extended Analysis}
In this section, we present a statistics to quantify various facets of patch generations following the metrics laid out in Table~\ref{table:quantitative-analysis-gens}.
In Table~\ref{table:quantitative-analysis-gens-all}, we recalculate these values for \textit{all} patch generations in the oracle retrieval setting for all models, regardless of whether or not the patch was applied successfully.
Across all metrics, we find that patch generations across models are much closer in size to the characteristics of average gold edits.
While some models still generate fewer lines relative to the corresponding Gold edit (e.g., Claude-2, ChatGPT-3.5, GPT-4), the SWE-Llama models edits are on average longer in most respects..
When considering both Table~\ref{table:quantitative-analysis-gens} and Table~\ref{table:quantitative-analysis-gens-all}, it becomes clear that models struggle with generating longer output sequences to be correctly formatted patches.
Further inspection of such occurrences, as shown in our case studies in Section~\ref{appx:extra-results:quality-in-depth}, indicate that hallucinations, abiding to existing code style/structure, and referencing long range dependencies correctly are common errors that surface more frequently in longer generations.

\input{tables/appx/quantiative-analysis-gens-all}

\subsection{Software Engineering Metrics}
We perform preliminary evaluations that explore using \textit{software engineering} metrics to evaluate the efficiency and complexity of large code blocks integrated within a complex codebase.
Unlike semantic similarity scoring functions for evaluating fluency and surface form likeness that are popular with traditional NLP benchmarks and have been adopted for code generation, metrics such as Cyclomatic complexity~\cite{mccabe1976complexity} and Halstead complexity measures~\cite{Halstead1977ElementsOS} are founded upon logical abstractions (e.g., Abstract Syntax Trees) and software principles to quantify the complexity, efficiency, and readability of code as a scalar value.
The patch generations and \benchmark{} evaluation logs are rich sources of information that software engineering metrics and static analyzers can readily be applied to.
Unlike small, code contest benchmarks where the insights of software engineering metrics are not meaningful due to the minuscule scope of the target functionality, \benchmark{}'s task is complex enough that practitioners can use these tools to gain well-structured, rigorous, and wide-ranging feedback signals on the complexity of a patch generation's change and its effect on the rest of the codebase.

\input{figures/swe-metrics-study}

We include our exploratory work here that demonstrates how software engineering metrics can reliably capture characteristics of code quality, and how comparing these statistics across two patches can provide automatic observations about model capabilities.
We use the Radon package\footnote{Radon \href{https://radon.readthedocs.io/en/latest/}{Documentation}, open-source \href{https://github.com/rubik/radon}{codebase}}, a library for computing different software engineering metrics directly from source code.

We look specifically at successfully applied Claude 2 patch predictions in the ``Oracle" retrieval setting for the \texttt{psf/requests} repository, which several models perform best at as reflected in Figure~\ref{fig:per-repo-oracle-fig}.
Per prediction, we apply the patch to the codebase, then calculate the Cyclomatic complexity and Halstead complexity scores for the modified functions.
Cyclomatic complexity quantifies the control flow of a function, counting the number of independent execution paths through the source code~\citep{mccabe1976complexity}.
A higher Cyclomatic complexity score suggests a more complex function that has higher likelihood of defects and usually suggests difficult maintainability.
Halstead complexity counts the number of operators and operands in a program~\citep{Halstead1977ElementsOS}.
Per prediction, we also perform the same set of steps for the corresponding gold patch.

We find that software engineering metrics provides automatic qualitative insights into model performance.
Consider the following simple case study in Figure~\ref{fig:swe-metrics-comparison}.
While the model patch prediction (left) is fewer lines ($6$ instead of $11$) and modifies fewer files ($1$ instead of $2$) compared to the gold reference solution (right), the model's edit places a conditional within a relatively complex and widely used \texttt{HTTPAdapter} class.
This introduces two new potential execution outcomes, raising the Cyclomatic complexity of \texttt{HTTPAdapter} from $3$ to $5$.
In contrast, while longer, the reference solution imports intra-module dependencies, modifies a logically simpler function in \texttt{get\_connection}, and defines a new error type \texttt{InvalidProxyURL} to capture the novel bug described by the issue.


==> appx/swe-llama.tex <==
\section{Additional Details on Training SWE-Llama}
\label{appx:swe-llama}

\subsection{Training Details}
\textbf{Optimization.} We finetune using LoRA~\citep{hu2022lora} with $r=16$, $\alpha=16$, $\text{dropout}=0.05$, on the query, key, value, and output projection matrices of every attention sublayer.
We train with a learning rate of $6e-4$ and a batch size of $32$ sequences per gradient step for a maximum of $4$ epochs.
During training, we save checkpoints every $50$ steps, and after training, select the best checkpoint based on the validation loss on a held-out $100$ instances.
\swellama{} 7b was initialized with CodeLlama-Python 7b and trained in $20$ hours on $4$ NVIDIA A100s.
\swellama{} 13b was initialized with CodeLlama-Python 13b and trained in $47$ hours on $8$ NVIDIA A100s.
We used DeepSpeed Ulysses~\citep{jacobs2023deepspeed} and Flash Attention~\citep{dao2022flashattention} to enable long context training.

==> figures/case-study.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/assets/case-study.pdf}
    \caption{
    We show an example of an formatted task instance, a model prediction, and the testing framework logs.
    In the patches, red highlights are deletions.
    Green highlights are additions.
    }
    \label{fig:case-study}
\end{figure}

==> figures/collection-pipeline.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/assets/construction-diagram.png}
    \caption{
    \benchmark{} task instances are created by taking an existing IaC repository and suggesting an initial example composed of prompt instruction, code block to mask, and unit tests. It then follows a series of optimizations via critic LLM that ensures the consistency of the code to the prompt instructions as well as difficulty of the example for LLMs. Once the example is optimized, it is benchmarked across state-of-the-art LLMs to validate its complexity.
    }
    \label{fig:collection-pipeline}
\end{figure}

==> figures/dataset-stats-cdfs.tex <==
\begin{figure}[htbp]
\centering

\begin{minipage}{0.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/assets/cdfs/p_num_words.png}
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/assets/cdfs/c_num_files.png}
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/assets/cdfs/c_num_lines.png}
\end{minipage}

\vspace{5pt}

\begin{minipage}{0.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/assets/cdfs/d_files_edited.png}
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/assets/cdfs/d_functions_edited.png}
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/assets/cdfs/d_lines_edited.png}
\end{minipage}

\vspace{5pt}

\begin{minipage}{0.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/assets/cdfs/t_num_f2p.png}
\end{minipage}
\hspace{5pt}
\begin{minipage}{0.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/assets/cdfs/t_num_p2p.png}
\end{minipage}

\caption{
Cumulative Distribution Functions for different attributes of \benchmark{} task instances.
}
\label{table:dataset-stats-cdfs}
\end{figure}

==> figures/dataset-stats.tex <==
\begin{table}[t]
\begin{minipage}{.49\linewidth}
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/assets/task-distribution.pdf}
        \captionof{figure}{
        [TO BE REPLACED] Distribution of \benchmark{} repos ...
        }
        \label{fig:task-distribution}
    \end{minipage}
\end{minipage}
\hfill
\begin{minipage}{.48\linewidth}
    \begin{minipage}{\textwidth}
        \centering
        \caption{
        [TO BE REPLACED] Statistics of \benchmark{} task instance...
        }
        \resizebox{\textwidth}{!}{
        \small
        \begin{tabular}{llrr}
        \toprule
            & & Mean & Max \\
        \midrule
            Issue Text & Length (Words) & 195.1 & 4477 \\
            \midrule
            \multirow{2}{*}{Codebase} & \# Files (non-test) & 3,010 & 5,890 \\
                                      & \# Lines (non-test) & 438K  & 886K \\
            \midrule
            \multirow{3}{*}{Gold Patch} & \# Lines edited & 32.8 & 5888 \\
                                        & \# Files edited & 1.7 & 31 \\
                                        & \# Func. edited & 3 & 36 \\
            \midrule
            \multirow{2}{*}{Tests} & \# Fail to Pass & 9.1 & 1633 \\
                                   & \# Total & 120.8 & 9459 \\
        \bottomrule
        \end{tabular}
        }
        \label{table:dataset-stats}
    \end{minipage}
\end{minipage}
\vspace{-0.5em}
\end{table}


==> figures/evaluation-pipeline.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/assets/pipeline-evaluation.pdf}
    \caption{
    Visualization of the evaluation pipeline at an individual task instance level.
    During evaluation, the \textit{Patch} is model generated.
    A prediction \texttt{.patch} must be applied successfully and produce the same results as the corresponding task instance's $D$ for task completion.
    }
    \label{fig:eval-pipeline}
\end{figure}

==> figures/per-repo-pass-rate.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/assets/per_repo_oracle_fig.pdf}
    \caption{
    Resolution rate for three models across the 12 repositories represented in \benchmark{} in the ``Oracle" retrieval setting.
    }
    \label{fig:per-repo-oracle-fig}
\end{figure}

==> figures/swe-metrics-study.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{p{0.9\linewidth}}
    \toprule
    \textbf{Problem Statement}: Misleading exception with invalid protocol in proxy variable. When the value of \texttt{https\_proxy} or \texttt{HTTPS\_PROXY} variable(s) accidentally miss one '/' in the protocol, a traceback is thrown to the user which doesn't pin point that the issue is with the proxy configuration... \\
    \bottomrule
    \vspace{1em}
\end{tabular}
\begin{minipage}{.44\linewidth}
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/assets/swe-metrics-pred.pdf}
    \end{minipage}
\end{minipage}
\hfill
\begin{minipage}{.55\linewidth}
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/assets/swe-metrics-gold.pdf}
    \end{minipage}
\end{minipage}
\captionof{figure}{Comparison of the Claude 2 prediction (left) and reference solution (right) patches for \benchmark{} task instance \texttt{psf\_\_requests-4356}. While the code generated by the patch is fewer lines of code and solves the problem correctly, the prediction patch introduces greater Cyclomatic complexity (\texttt{requests.adapters.py/HTTPAdapter}: 3 $\rightarrow$ 5) compared to the gold solution (\texttt{requests/adapters.py:get\_connection}: 2 $\rightarrow$ 3, \texttt{requests/exceptions.py:InvalidHeader}: 0 $\rightarrow$ 1). Changes that introduce new execution paths are boxed in blue. Parts of the gold patch have been truncated for appearance.}
\label{fig:swe-metrics-comparison}
\end{table}


==> figures/swellama-correct-context-length-vs-test.tex <==
\begin{figure}[!htb]
\begin{minipage}{0.64\linewidth}
    \centering
    \includegraphics[width=0.98\textwidth]{figures/assets/swellama-issue-length-tokens.pdf}
    \captionof{figure}{We compare the performance of Claude 2 on tasks partitioned by total input length and by only the issue length.}
    \label{fig:performance-vs-context-length}
\end{minipage}%
\hfill
\begin{minipage}{0.34\linewidth}
\captionof{table}{We show the results for the ``Oracle"-collapsed retrieval setting, which uses oracle files but collapses code that isn't directly modified by the PR $\pm 15$  lines.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcc}
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{2}{c}{``Oracle"-collapsed} \\
    \cmidrule(lr){2-3}
    & Resolved & Applied \\
    \midrule
    Claude 3 Opus & {\bf 9.39} & 48.00       \\
    Claude 2      & 5.93       & {\bf 68.18} \\
    GPT-4         & 3.40       & 48.65       \\
    ChatGPT-3.5   & 1.09       & 40.93       \\
    \bottomrule
\end{tabular}
}
\label{table:editonly-results}
\end{minipage}
\end{figure}


==> figures/zero-shot-models-result.tex <==
\begin{figure}[H]
\centering
\includegraphics[width=0.95\textwidth]{figures/assets/general_models_results.pdf}
\caption{
One-attempt models correctness on \benchmark{} - average share of fully solved tasks
}
\label{fig:zero-shot-correctness}
\end{figure}

==> section/acknowledge.tex <==
\section*{Acknowledgements}
We thank Danqi Chen, Tri Dao, Zexuan Zhong, Tianyu Gao, Will Merrill, Mengzhou Xia, Dan Friedman, Adithya Bhaskar, Austin Watkins, Aatmik Gupta, and Richard Zhu for their valuable feedback and advice.
We acknowledge support from the National Science Foundation under Grant No. 2239363 and an Oracle Collaborative Research award.
Any opinions, findings, conclusions, or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.

==> section/customer_problem_statement.tex <==
\section*{Customer Problem Statement}
\label{sec:customer_statement}

This paper addresses a critical challenge faced by organizations that develop and maintain cloud infrastructure: complexity and technical expertise required for IaC development. Large-scale AWS customers such as Booking.com, Zalando, Volkswagen, and others extensively rely on AWS CDK for their pipelines and face considerable overhead in managing their cloud resources through code. Development teams must navigate intricate service dependencies, security configurations, and cloud-specific knowledge, often requiring specialized cloud engineering teams and documentation review.

Our benchmark directly benefits these customers by accelerating the advancement of AI assistants capable of understanding and modifying cloud infrastructure code. Improved LLM capabilities in this domain could significantly reduce development time, lower the barrier to entry for IaC adoption, and enable developers to focus on higher-level architectural decisions rather than implementation details. For enterprise customers with complex multi-service architectures, even incremental improvements in automation translate to substantial productivity gains and reduced operational errors. While some concerns exist about the changing role of cloud specialists with increasing automation, the AI tools are designed to augment developers' capabilities rather than replace them. Furthermore, any risks associated with automated IaC generation, including potential security vulenrabilities and resource misconfigurations are effectively mitigated through standard DevOps practices including code review, testing, and staged deployments.


==> section/experiments.tex <==
\section{Experimental Setup}
\label{sec:experimental-setup}
In this section we explain how inputs are constructed to run \benchmark{} evaluation.
In addition, we review the models that we evaluate in this work.

\subsection{Retrieval-Based Approach}
\label{sec:experimental-setup:input-formulation}
\benchmark{} instances provide an issue description and a codebase as input to the model.
While issues descriptions are usually short ($195$ words on average as shown in Table~\ref{table:dataset-stats}), codebases consist of many more tokens ($438$K lines on average) than can typically be fit into an LMs context window.
Then the question remains of exactly how to choose the relevant context to provide to the model?

To address this issue for our baselines, we simply use a generic retrieval system to select the files to insert as context.
In particular, we evaluate models under two relevant context settings: 1) sparse retrieval and 2) an oracle retrieval.

\textbf{Sparse retrieval.}
Dense retrieval methods are ill-suited to our setting due to very long key and query lengths, and especially the unusual setting of retrieving code documents with natural language queries.
Therefore, we choose to use BM25 retrieval~\citep{robertson2009probabilistic} to retrieve relevant files to provide as context for each task instance.
We experiment with three different maximum context limits, and simply retrieve as many files as fits within the specified limit.
We evaluate each model on all limits that fit within its context window and report the best performance.
From observation, models perform best on the shortest context window, as shown in Table~\ref{table:bm25-results}.

\textbf{``Oracle'' retrieval.}
For analysis purposes we also consider a setting where we ``retrieve'' the files edited by the reference patch that solved the issue on GitHub.
This ``oracle" setting is less realistic, since an engineer working on addressing an issue may not know a priori which files need to be modified.
In addition, this setting is also not necessarily comprehensive since edited files alone may not include all the required context to understand exactly how software will behave when interacting with unseen parts of the code.

We compare the BM25 retrieval results with those of the ``oracle'' retrieval setting, as shown in Table~\ref{table:recall}.
We observe that in approximately $40\%$ of instances, BM25 retrieves a superset of the oracle files for the $\num{27000}$-token context limit. However, in almost half of the instances with the $\num{27000}$-token limit, it retrieves none of the files from the ``oracle'' context.

\subsection{Input Format}
\label{sec:experimental-setup:input-format}
Once the retrieved files are selected using one of the two methods above, we construct the input to the model consisting of task instructions, the issue text, retrieved files and documentation, and finally an example patch file and prompt for generating the patch file.
Examples of instances and further details on this formulation are provided in Appendix~\ref{appx:experiment-details}.

\subsection{Models}
\label{sec:experimental-setup:models}
Due to the need to process long sequence lengths, there are only a few models that are currently suitable for  \benchmark{}.
Thus we evaluate ChatGPT-3.5 ({\small \texttt{gpt-3.5-turbo-16k-0613}}), GPT-4 ({\small \texttt{gpt-4-32k-0613}}), Claude 2, and \swellama{} with their context limits shown in Table~\ref{tab:model-context-comparision}.

\input{tables/bm25-results}

\input{tables/model-context-comparision}


==> section/statements.tex <==
\section{Ethics Statement}
\label{sec:ethics-statement}

\benchmark{} is collected entirely from public repositories with licenses that permit software usage that our contributions are in accordance with.
Details of the licenses are included in Table~\ref{table:repo-summaries}.
During the collection or evaluation processes, we do not collect information about GitHub users, and the \benchmark{} task instances do not use GitHub data beyond what is offered via the public API and website.
Our contributions do not involve any human subject participation; we do not perform crowdsourcing or recruit human task workers for any part of \benchmark{}, including its collection and evaluation procedures along with the experiments.
\benchmark{}'s filtering criteria for GitHub repositories based on popularity does not implicitly or explicitly rely on any discriminative or biased heuristics for repository selection.
For the dataset release, we plan to open source the \benchmark{} task instances, the collection and evaluation infrastructure, the experimental results, the training data used for fine-tuning \swellama{} models, and the \swellama{} model weights.
Following best practice precedents, we will also put forth ample documentation to describe each component and its use, and we will also put in place convenient communication channels for soliciting feedback to improve \benchmark{}.
\benchmark{} does not put forth any immediately harmful insights.
We briefly discuss the potential impact of \benchmark{}'s usage in Section~\ref{appx:societal-impact}.

\section{Reproducibility Statement}
\label{sec:reproducibility-statement}
For our submission, we have uploaded the entirety of the source code as a zipped file that has been properly anonymized.
We have organized the codebase such that separate directories correspond to different contributions within the main paper (i.e. dataset collection, evaluation, open source model inference, \swellama{} training, etc.).
The source code contains inline documentation that details purpose and usage of different parts of the codebase.
In addition, we also include the full set of 2294 \benchmark{} task instances that contains all the components discussed in the main paper.
Beyond the documentation in the source code, we include thorough technical details for the collection pipeline and evaluation procedures in Section~\ref{appx:benchmark:construction} and Section~\ref{appx:benchmark:eval-procedure} that complements the original details in Section~\ref{sec:benchmark} of the main paper.
These sections fully cover the logic presented in the code and can be helpful for understanding it.
Moving forward, as discussed in the ethics statement, we plan to more formally release \benchmark{} to the public as an open source repository with thorough details that describes the benchmark, outlines the code, and details its usage.
A major component of \benchmark{} is the collection framework, which will be part of the open sourced code.
Because of its easily maintainable design, as discussed in the main paper, our hope and belief is that \benchmark{} should be highly reproducible.


==> section/swe-llama.tex <==
\section{\swellama{}: Fine-tuning CodeLlama for \benchmark{}}
\label{sec:swellama-fine-tuning-codellama-for-benchmark}

It is important to benchmark the performance of open models on \benchmark{} alongside proprietary models.
At the time of writing, only the CodeLlama models~\citep{rozière2023code} are able to handle the very long contexts necessary.
However, we observe that the off-the-shelf CodeLlama variants are not capable of following the detailed instructions to generate repository-wide code edits, and typically output placeholder responses or unrelated code. To better evaluate the capabilities of these models, we perform supervised fine-tuning on the $7$ billion- and $13$ billion-parameter CodeLlama-Python models. The resulting models are specialized repository editors that can run on consumer hardware and resolve GitHub issues.

\textbf{Training data.} We follow our data collection procedure and collect $\num{19000}$ issue-PR pairs from an additional 37 popular Python package repositories. In contrast to Section~ \ref{sec:benchmark:construction}, we do not require that pull requests contribute test changes.
This allows us to create a much larger training set to use for supervised fine-tuning.
To eliminate the risk of data contamination, the set of repositories in the training data is disjoint from those included in the evaluation benchmark.

\textbf{Training details.}  
Given the instructions, an issue text from GitHub and the relevant code files as the prompt, we finetune \swellama{} to generate the patch that solved the given issue (the ``gold patch'').
For memory efficiency, we fine-tune only the weights of the attention sublayer using LoRA~\cite{hu2022lora}, and exclude training sequences with more than $\num{30000}$ tokens, reducing the effective size of the training corpus to $\num{10000}$ instances. More details are provided in Appendix \ref{appx:swe-llama}.

==> tables/appx/dev-issue-tags.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{l|ll}
\toprule
    Category & Count & Examples \\
\midrule
    Bug & 127 & ``bug" (111); ``Bug :cockroach:" (10); ``rule bug" (6); \\
    Feature & 55 & ``enhancement": 46; ``Enhancement :star:": 5; ``feature-request": 2; \\
    Regression & 4 & ``Regression" (4); \\
    Other & 95 & ``api": 11, ``documentation": 7, ``help wanted": 6, ``config options": 5, \\
          &    & ``io": 5, ``jinja": 4, ``good first issue": 4, ``parser" 3 \\
\bottomrule
\end{tabular}
\caption{Categories of tags associated with issues from \benchmark{}'s development task instances.}
\label{table:dev-issue-tags}
\end{table}

==> tables/appx/dev-repo-dataset-stats.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{l|llllllllllll}
    \toprule
        & astroid & marshmallow & pvlib & pydicom & pyvista & sqlfluff \\
    \midrule
        $P$ Length (Characters)        & $2199$ & $1619$ & $1790$ & $2076$ & $1475$ & $2639$ \\
        $C$ \# Files                   & $252$ & $82$ & $294$ & $455$ & $866$ & $2297$ \\
        $C$ \# Lines                   & $60$K & $22$K & $459$K & $170$K & $661$K & $205$K \\
        $\delta$ \# Files Edited       & $2.51$ & $1.89$ & $1.83$ & $1.54$ & $2.1$ & $3.26$ \\
        $\delta$ \# Func. Edited       & $3.03$ & $2.11$ & $2.89$ & $2.23$ & $3.0$ & $2.71$ \\
        $\delta$ \# Lines Edited       & $83.1$ & $36.2$ & $93.3$ & $42.0$ & $101.0$ & $102.5$ \\
        $\delta$ \# Lines Added        & $52.8$ & $24.7$ & $67.0$ & $29.7$ & $79.4$ & $63.6$ \\
        $\delta$ \# Lines Removed      & $30.3$ & $11.6$ & $26.4$ & $12.3$ & $21.6$ & $38.9$ \\
        $\vert T \vert$ (Fail to Pass) & $23.2$ & $53.0$ & $19.1$ & $24.0$ & $8.8$ & $14.8$ \\
        $\vert T \vert$ (Pass to Pass) & $182.6$ & $242.9$ & $107.5$ & $176.1$ & $96.5$ & $239.7$ \\
        $\vert T \vert$ (All)          & $205.8$ & $295.9$ & $126.6$ & $200.1$ & $105.3$ & $254.5$ \\
    \bottomrule
\end{tabular}
\caption{Average numbers characterizing different attributes of a \benchmark{} task instance grouped by repository for repositories in the development dataset. The same statistics presented in Table~\ref{table:repo-dataset-stats} are also shown here.}
\label{table:dev-repo-dataset-stats}
\end{table}

==> tables/appx/dev-repo-summaries.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{l|lcl}
\toprule
    Repository & Summary & Count & License \\
\midrule
    marshmallow-code/  & Parse complex objects to/from Python data-types & 9 & MIT \\
    \quad marshmallow  & & & \\
    pylint-dev/astroid & Library for AST parsing, static analysis/inference & 31 & LGPL-2.1 \\
    pydicom/pydicom    & Read/modify/write DICOM files w/ Python & 56 & Custom \\
    pvlib/pvlib-python & Simulate photovoltaic energy systems performance & 63 & Custom \\
    pyvista/pyvista    & 3D plotting, mesh analysis through interface & 16 & MIT \\
    sqlfluff/sqlfluff  & SQL linter, supports multiple dialects, templates & 50 & MIT \\
\bottomrule
\end{tabular}
\caption{Summary and licenses for all GitHub repositories that development task instances were extracted from.}
\label{table:dev-repo-summaries}
\end{table}

==> tables/appx/issue-tags.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{l|ll}
\toprule
    Category & Count & Examples \\
\midrule
    Bug & 442 & ``Bug" (179); ``type:bug" (114); ``bug" (57); ``type: bug" (48); \\
        & & ``Bug :beetle:" (23); ``status: confirmed bug" (20);; \\
    Feature & 167 & ``type:enhancement" (47); ``Enhancement" (25); ``New feature" (24); \\
        & & ``Feature Request" (22); ``type: enhancement" (19); \\
        & & ``Enhancement :star:" (15); ``New Feature" (7); ``enhancement" (6);  \\
    Regression & 39 & ``type: regression" (14); ``Regression" (14); ``regression" (8); \\
    Other & 1641 & ``help wanted" (71); ``good first issue" (66); ``printing" (58); \\
        & & ``extensions:autodoc" (58); ``Easy" (57); ``Easy to Fix" (54); \\
        & & ``domains:py" (27); ``core" (26); ``sets" (23); ``Wrong Result" (23); \\
        & & ``units" (22); ``Good first issue" (21); \\
\bottomrule
\end{tabular}
\caption{Categories of tags associated with issues from \benchmark{}'s task instances.}
\label{table:issue-tags}
\end{table}

==> tables/appx/main-results-20.tex <==
\definecolor{forestgreen}{RGB}{52,194,48}

\begin{table}[ht]
\centering
\begin{tabular}{lrrrr}
\toprule
\multirow{2}{*}{} & \multicolumn{2}{c}{BM25 Retrieval} & \multicolumn{2}{c}{``Oracle'' Retrieval} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} 
Model & \% Resolved & \multicolumn{1}{c}{\% Apply} & \% Resolved & \% Apply  \\
\midrule
Claude 2       & 2.27 \textcolor{forestgreen}{$\uparrow 0.31$} & 45.72 \textcolor{forestgreen}{$\uparrow 2.65$} & 4.01 \textcolor{red}{$\downarrow 0.79$} & 62.65 \textcolor{red}{$\downarrow 0.17$} \\
ChatGPT-3.5    & 0.17 \textcolor{gray}{$- 0.00$} & 26.53 \textcolor{forestgreen}{$\uparrow 0.02$} & 0.70 \textcolor{forestgreen}{$\uparrow 0.18$} & 21.64 \textcolor{red}{$\downarrow 0.16$} \\
GPT-4          & 0.00 \textcolor{gray}{$- 0.00$} & 14.82 \textcolor{gray}{$- 0.00$} & 1.74 \textcolor{gray}{$- 0.00$} & 34.00 \textcolor{gray}{$- 0.00$} \\
SWE-Llama 7b   & 0.35 \textcolor{forestgreen}{$\uparrow 0.35$} & 49.04 \textcolor{red}{$\downarrow 2.70$} & 1.92 \textcolor{red}{$\downarrow 1.09$} & 63.70 \textcolor{red}{$\downarrow 1.82$} \\
SWE-Llama 13b  & 0.70 \textcolor{gray}{$- 0.00$} & 56.54 \textcolor{forestgreen}{$\uparrow 2.92$} & 4.54 \textcolor{forestgreen}{$\uparrow 0.57$} & 66.67 \textcolor{red}{$\downarrow 0.11$} \\

\bottomrule
\end{tabular}
\caption{
We compare models against each other using the BM25 and oracle retrieval settings as described in Section~\ref{sec:experimental-setup} on a $25$\% random subset (574 instances) of \benchmark{} in the ``oracle" and BM25 27K retriever settings only. This is the same subset that GPT-4 is evaluated on, as mentioned in Table~\ref{table:main-results}. The difference relative to percentages in Table~\ref{table:main-results} and Table~\ref{table:main-results-oracle} is included as a subscript.
}
\label{table:main-results-20}
\end{table}

% \textcolor{forestgreen}{$\uparrow 0.31$}
% \textcolor{red}{$\downarrow 2.46$}
% \textcolor{gray}{$- 0.00$}

==> tables/appx/main-results-repo.tex <==
\begin{table}[ht]
\begin{tabular}{lrrrrr}
    \toprule
    Repo & Claude 2 & ChatGPT-3.5 & GPT-4 & SWE-Llama $13$b & SWE-Llama $7$b \\
    \midrule
    astropy/astropy           & \num{3.23}  & \num{0.00} & \num{0.00} & \num{1.06 } & \num{3.16 } \\
    django/django             & \num{6.15}  & \num{1.32} & \num{2.50} & \num{5.19 } & \num{4.00 } \\
    matplotlib/matplotlib     & \num{3.05}  & \num{3.33} & \num{0.00} & \num{3.12 } & \num{1.11 } \\
    mwaskom/seaborn           & \num{0.00}  & \num{0.00} & \num{0.00} & \num{0.00 } & \num{0.00 } \\
    pallets/flask             & \num{0.00}  & \num{0.00} & \num{0.00} & \num{9.09 } & \num{0.00 } \\
    psf/requests              & \num{15.91} & \num{2.33} & \num{8.33} & \num{13.64} & \num{18.18} \\
    pydata/xarray             & \num{6.90}  & \num{0.00} & \num{0.00} & \num{5.81 } & \num{3.00 } \\
    pylint-dev/pylint         & \num{1.75}  & \num{0.00} & \num{0.00} & \num{1.75 } & \num{1.75 } \\
    pytest-dev/pytest         & \num{5.93}  & \num{0.00} & \num{0.00} & \num{5.04 } & \num{4.20 } \\
    scikit-learn/scikit-learn & \num{5.41}  & \num{0.00} & \num{0.00} & \num{3.12 } & \num{0.88 } \\
    sphinx-doc/sphinx         & \num{5.65}  & \num{1.83} & \num{0.00} & \num{2.25 } & \num{2.69 } \\
    sympy/sympy               & \num{1.94}  & \num{0.00} & \num{0.00} & \num{3.01 } & \num{1.59 } \\
    \bottomrule
\end{tabular}
\caption{\% Resolved for models per repository represented in \benchmark{}.}
\label{table:main-results-repo}
\end{table}

==> tables/appx/oracle-results.tex <==
\begin{table}
\centering
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{} & \multicolumn{2}{c}{``Oracle'' Retrieval} \\
\cmidrule(lr){2-3} 
Model & \% Resolved & \% Apply  \\
\midrule
Claude 2        & {\bf 4.80} & 62.82  \\
ChatGPT-3.5     & 0.52       & 21.80  \\
GPT-4$^*$       & 1.74       & 34.00  \\
SWE-Llama 7b    & 3.01       & 65.52  \\
SWE-Llama 13b   & 3.97       & {\bf 66.78}  \\
\bottomrule
\end{tabular}
\caption{
We compare models against each other using the oracle retrieval settings as described in Section~\ref{sec:experimental-setup}. The main results table, Table~\ref{table:main-results}, presents the results for the different models when using BM25 only. $^*$Due to budget constraints we evaluate GPT-4 on a $25$\% random subset of \benchmark{} in the ``Oracle" and BM25 27K retriever settings only.
}
\label{table:main-results-oracle}
\end{table}


% \begin{table}
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \multirow{2}{*}{} & \multicolumn{2}{c}{BM25 Retrieval} & \multicolumn{2}{c}{``Oracle'' Retrieval} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
% Model & \% Resolved & \% Apply  & \% Resolved & \% Apply  \\
% \midrule
% Claude 2        & {\bf 1.96} & 43.07       & {\bf 4.80} & 62.82  \\
% ChatGPT-3.5     & 0.17       & 26.33       & 0.52       & 21.80  \\
% GPT-4$^*$       & 0.00       & 14.83       & 1.74       & 34.00  \\
% SWE-Llama 7b    & 0.70       & 51.74       & 3.01       & 65.52  \\
% SWE-Llama 13b   & 0.70       & {\bf 53.62} & 3.97       & {\bf 66.78}  \\
% \bottomrule
% \end{tabular}
% \caption{
% We compare models against each other using the BM25 and oracle retrieval settings as described in Section~\ref{sec:experimental-setup}. The main results table, Table~\ref{table:main-results}, presents the results for the different models when using BM25 only. $^*$Due to budget constraints we evaluate GPT-4 on a $25$\% random subset of \benchmark{} in the ``Oracle" and BM25 27K retriever settings only.
% }
% \label{table:main-results-oracle}
% \end{table}


==> tables/appx/patch-fix-rates.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{llcccc}
\toprule
    Model & Retrieval Setting & Generations & Applies & Fixed & Patch Fix \% \\
\midrule
    ChatGPT-3.5   & BM25 $13$k            & \num{2270} & \num{604} & \num{363} & \num{60.1}\%  \\
    ChatGPT-3.5   & ``Oracle''            & \num{1262} & \num{500} & \num{222} & \num{44.4}\%  \\
    ChatGPT-3.5   & ``Oracle''-collapsed  & \num{1811} & \num{939} & \num{420} & \num{44.73}\%  \\
    Claude 2      & BM25 $13$k            & \num{2281} & \num{988} & \num{302} & \num{30.57}\%  \\
    Claude 2      & ``Oracle''            & \num{2138} & \num{1441} & \num{360} & \num{24.98}\%  \\
    Claude 2      & ``Oracle''-collapsed  & \num{2242} & \num{1564} & \num{465} & \num{29.73}\%  \\
    GPT-4         & BM25 $27$k            & \num{573} & \num{85} & \num{59} & \num{69.41}\%  \\
    GPT-4         & ``Oracle''            & \num{462} & \num{195} & \num{121} & \num{62.05}\%  \\
    GPT-4         & ``Oracle''-collapsed  & \num{2292} & \num{1116} & \num{684} & \num{61.29}\%  \\
    SWE-Llama 13b & BM25 $13$k            & \num{2010} & \num{1230} & \num{369} & \num{30.0}\%  \\
    SWE-Llama 13b & ``Oracle''            & \num{2125} & \num{1532} & \num{378} & \num{24.67}\%  \\
    SWE-Llama 7b  & BM25 $13$k            & \num{2139} & \num{1187} & \num{340} & \num{28.64}\%  \\
    SWE-Llama 7b & ``Oracle''             & \num{2119} & \num{1503} & \num{298} & \num{19.83}\%  \\
\bottomrule
\end{tabular}
\caption{Statistics for how many patches for $\num{2294}$ task instances were generated, applied successfully, and required a post-generation fix to apply successfully for each [model, retrieval setting] combination during evaluation. The GPT-4 BM25 27k and ``Oracle" settings were ran on the 25\% subset. The GPT-4 ``Oracle"-collapsed setting was run on the full \benchmark{} test set.}
\label{table:patch-fix-rates}
\end{table}

==> tables/appx/quantiative-analysis-gens-all.tex <==
\begin{table}[ht]
\centering
\caption{
Average edits of model generated patches in the oracle retrieval setting across all patches (including unsuccessfully applied patches).
For the task instances specific to each model, we calculate the same statistics across the gold patches.
}
\begin{tabular}{lccccc}
\toprule
    Model & Total Lines & Added & Removed & Functions & Files \\ \cmidrule(lr){1-1} \cmidrule(lr){2-6}  
    Claude 2 & 27.2 & 6.6 & 3.3 & 1.2 & 1.1 \\
    \quad Gold & 61.6 & 17.8 & 8.6 & 2.6 & 1.4 \\
\midrule
    ChatGPT-3.5 & 42.0 & 6.1 & 3.9 & 1.7 & 1.0 \\
    \quad Gold & 44.5 & 12.7 & 5.5 & 2.1 & 1.2 \\
\midrule
    GPT-4 & 22.4 & 4.4 & 1.8 & 0.8 & 0.9 \\
    \quad Gold & 50.3 & 14.0 & 6.5 & 2.3 & 1.3 \\
\midrule
    SWE-Llama 13b & 68.9 & 9.5 & 4.3 & 2.5 & 1.6 \\
    \quad Gold & 61.5 & 17.8 & 8.6 & 2.6 & 1.4 \\
\midrule
    SWE-Llama 7b & 78.9 & 10.1 & 7.6 & 2.5 & 1.5 \\
    \quad Gold & 65.1 & 18.8 & 9.0 & 2.7 & 1.5 \\
\bottomrule
\end{tabular}
\label{table:quantitative-analysis-gens-all}
\end{table}

==> tables/appx/repo-conversion-stats.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{l|lll}
\toprule
    Repo & Total PRs Crawled & Post-Conversion & Post-Validation (Final) \\
\midrule
    astropy & \num{9469} & \num{1016} & \num{95} \\
    django & \num{16914} & \num{2880} & \num{850} \\
    flask & \num{2434} & \num{107} & \num{11} \\
    matplotlib & \num{16545} & \num{1057} & \num{184} \\
    pylint & \num{3848} & \num{787} & \num{57} \\
    pytest & \num{5147} & \num{750} & \num{119} \\
    requests & \num{2344} & \num{84} & \num{44} \\
    scikit-learn & \num{15159} & \num{1169} & \num{229} \\
    seaborn & \num{1004} & \num{203} & \num{22} \\
    sphinx & \num{4931} & \num{645} & \num{187} \\
    sympy & \num{11928} & \num{1897} & \num{386} \\
    xarray & \num{3416} & \num{812} & \num{110} \\
\midrule
    Total & \num{93139} & \num{11407} & \num{2294} \\
\bottomrule
\end{tabular}
\caption{Statistics for how many candidate task instances were kept after the completion of a stage across the construction and validation procedures.}
\label{table:repo-conversion-stats}
\end{table}

==> tables/appx/repo-dataset-stats.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{l|llllllllllll}
    \toprule
        & astropy & django & flask & matplotlib & pylint & pytest \\
    \midrule
        $P$ Length (Characters)        & \num{2742} & \num{1307} & \num{1185} & \num{2381} & \num{2011} & \num{2948} \\
        $C$ \# Files                   & \num{1811} & \num{6356} & \num{225}  & \num{4395} & \num{2426} & \num{497}  \\
        $C$ \# Lines                   & \num{804}k & \num{407}k & \num{35}k  & \num{646}k & \num{109}k & \num{111}k \\
        $\delta$ \# Files Edited            & \num{1.5} & \num{1.5} & \num{1.6} & \num{1.5} & \num{1.8} & \num{1.4} \\
        $\delta$ \# Func. Edited           & \num{2.5} & \num{2.0} & \num{2.4} & \num{2.2} & \num{1.8} & \num{1.7} \\
        $\delta$ \# Lines Edited            & \num{36.0} & \num{18.5} & \num{35.4} & \num{58.9} & \num{36.0} & \num{24.5} \\
        $\delta$ \# Lines Added             & \num{25.0} & \num{12.8} & \num{23.7} & \num{35.7} & \num{26.6} & \num{18.2} \\
        $\delta$ \# Lines Removed           & \num{10.9} & \num{5.7}  & \num{11.6} & \num{23.2} & \num{9.5}  & \num{6.4}  \\
        $\vert T \vert$ (Fail to Pass) & \num{21.7} & \num{8.8}  & \num{1.4}  & \num{2.4}  & \num{6.8}  & \num{4.1}  \\
        $\vert T \vert$ (Pass to Pass) & \num{191.0} & \num{85.9} & \num{32.5} & \num{242.4} & \num{47.0} & \num{60.7} \\
        $\vert T \vert$ (All)          & \num{212.8} & \num{94.6} & \num{33.9} & \num{244.8} & \num{53.7} & \num{64.8} \\


    \midrule
        & requests & scikit-learn & seaborn & sphinx & sympy & xarray \\
    \midrule
$P$ Length (Characters)        & \num{1654} & \num{2239} & \num{1667} & \num{1888} & \num{1213} & \num{3515}  \\
$C$ \# Files                   & \num{119} & \num{1224} & \num{273}  & \num{1483} & \num{1666} & \num{260}   \\
$C$ \# Lines                   & \num{30}k  & \num{361}k & \num{105}k & \num{423}k & \num{678}k & \num{137}k  \\
$\delta$ \# Files Edited       & \num{1.64} & \num{1.68} & \num{1.77} & \num{1.51} & \num{1.9}  & \num{2.45}  \\
$\delta$ \# Func. Edited       & \num{1.59} & \num{2.24} & \num{1.41} & \num{2.72} & \num{3.22} & \num{3.16} \\
$\delta$ \# Lines Edited       & \num{25.5} & \num{44.0} & \num{30.1} & \num{30.6} & \num{36.3} & \num{124.8} \\
$\delta$ \# Lines Added        & \num{19.2} & \num{32.7} & \num{24.9} & \num{22.0} & \num{24.2} & \num{95.6}  \\
$\delta$ \# Lines Removed      & \num{6.2}  & \num{11.3} & \num{5.2}  & \num{8.6}  & \num{12.1} & \num{29.2}  \\
$\vert T \vert$ (Fail to Pass) & \num{7.6}  & \num{7.5}  & \num{12.9} & \num{2.3}  & \num{2.2}  & \num{58.5} \\
$\vert T \vert$ (Pass to Pass) & \num{87.1} & \num{150.7} & \num{86.8} & \num{45.1} & \num{74.5} & \num{297.5} \\
$\vert T \vert$ (All)          & \num{94.7} & \num{158.2} & \num{99.7} & \num{47.4} & \num{76.8} & \num{356.1} \\

    \bottomrule
\end{tabular}
\caption{Average numbers characterizing different attributes of a \benchmark{} task instance grouped by repository. In addition to the statistics presented in Table~\ref{table:dataset-stats}, we also introduce three new values: $\delta$ \# Lines Added, $\delta$ \# Lines Removed, and $\vert T \vert$ (Pass to Pass).}
\label{table:repo-dataset-stats}
\end{table}

==> tables/appx/repo-summaries.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{l|ll}
\toprule
    Repository & Summary & License \\
\midrule
    astropy/astropy & Astronomy and astrophysics core library & BSD 3-Clause \\
    django/django & Web framework for building web applications & BSD 3-Clause \\
    pallets/flask & Lightweight framework for small web apps & BSD 3-Clause \\
    matplotlib/matplotlib & Plotting library for creating visuals & Custom \\
    pylint-dev/pylint & Static code analyser for Python 2 or 3 & GPL 2.0 \\
    pytest-dev/pytest & Testing framework for Python & MIT \\
    psf/requests & Simple, elegant library for writing HTTP requests & Apache-2.0 \\
    scikit-learn/scikit-learn & Machine Learning in Python & BSD 3-Clause \\
    mwaskom/seaborn & Statistical data visualization in Python & BSD 3-Clause \\
    sphinx-doc/sphinx & Library for creating documentation & Custom \\
    sympy/sympy & Computer algebra system written in Python & Custom \\
    pydata/xarray & N-D labeled arrays and datasets & Apache-2.0 \\
\bottomrule
\end{tabular}
\caption{Summary and licenses for all GitHub repositories that task instances were extracted from.}
\label{table:repo-summaries}
\end{table}

==> tables/appx/six-outcome-cases.tex <==
\definecolor{green1}{RGB}{3,102,8}
\definecolor{green2}{RGB}{37,141,40}
\definecolor{green3}{RGB}{82,198,85}
\definecolor{green4}{RGB}{102,221,160}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|ccc}
    \toprule
            & \multicolumn{3}{c}{\# F2P Tests Pass} \\
    \cmidrule(lr){2-4} 
    \# P2P Tests Pass & All               & Partial            & None \\
    \midrule
        All & \textcolor{green1}{Resolved} & \textcolor{green3}{Partially Resolved} & No-Op  \\
    Partial & \textcolor{green2}{Breaking Resolved} & \textcolor{green4}{Work in Progress} & \textcolor{red}{Regression} \\
       None & \textcolor{green2}{Breaking Resolved} & \textcolor{green4}{Work in Progress} & \textcolor{red}{Regression} \\
    \bottomrule
    \end{tabular}
    \caption{We present the 6 possible outcomes for a patch generation that is applied successfully and then executed. The outcomes are distinguished by the number of F2P and P2P tests that pass.}
    \label{table:six-outcome-cases}
\end{table}


==> tables/appx/six-outcome-stats.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{l|ccccc}
    \toprule
Model & Claude 2 & ChatGPT-3.5 & GPT-4$^*$ & SWE-Llama 7b & SWE-Llama 13b \\
    \midrule
Applied & 1078 & 284 & 76 & 1257 & 1196 \\
    \midrule
\textcolor{green1}{Resolved} & 110 & 12 & 10 & 69 & 91 \\
\textcolor{green2}{Breaking Resolved} & 26 & 2 & 3 & 17 & 10 \\
\textcolor{green3}{Partially Resolved} & 15 & 4 & 3 & 17 & 10 \\
\textcolor{green4}{Work in Progress} & 20 & 2 & 1 & 17 & 16 \\
No-Op & 471 & 174 & 30 & 716 & 672 \\
\textcolor{red}{Regression} & 436 & 90 & 29 & 421 & 397 \\
    \bottomrule
    \end{tabular}
    \caption{Categorization of model generations that applied successfully by the cases defined in Table~\ref{table:six-outcome-cases}. As mentioned, GPT-4 was evaluated on a $25$\% subset (574 instances) of \benchmark{}.}
    \label{table:six-outcome-stats}
\end{table}

==> tables/appx/task-instance-fields.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{l|ll}
\toprule
    Field & Description \\
\midrule
    \texttt{base\_commit} & (str) The commit ID that the original PR is applied on top of \\
    \texttt{created\_at} & (date) Datetime object of when PR was first created (not merged) \\
    \texttt{hints\_text} & (str) Natural language suggestions for how to solve problem \\
    \texttt{instance\_id} & (str) A unique identifier created from \texttt{repo} and \texttt{pull\_number} \\
    \texttt{issue\_numbers} & (list) List of issue numbers that the original pull request resolves\\
    \texttt{patch} & (str) \texttt{.patch}-format styled string that is a reference solution \\
        & to the problem, extracted from the original PR's code changes \\
    \texttt{problem\_statement} & (str) Natural language description of desired change to codebase \\
    \texttt{pull\_number} & (int) The pull number of the original pull request \\
    \texttt{test\_patch} & (str) \texttt{.patch}-format styled string containing unseen tests \\
        & for checking if a task was solved, extracted from the original \\
        & PR's code changes \\
    \texttt{version} & (str) Release version (w.r.t. \texttt{repo}) during which PR was created \\
    \texttt{repo} & (str) The repository the task instance originates from \\
    \texttt{FAIL\_TO\_PASS} & (list) List of tests that change in status from \textit{fail} to \textit{pass} \\
    \texttt{PASS\_TO\_PASS} & (list) List of tests that change in status from \textit{pass} to \textit{pass} \\
    \texttt{env\_install\_commit} & (str) Base commit at which to install necessary \\ & dependencies for running task instance. \\
\bottomrule
\end{tabular}
\caption{Description of each field of a \benchmark{} task instance object. See \S~\ref{appx:benchmark:construction} for details regarding how each field is collected.}
\label{table:task-instance-fields}
\end{table}

==> tables/appx/temporal-results-extended.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc|ccccc}
\toprule
    Year & Total & 25\% & Claude 2 & GPT-3.5 & GPT-4$^*$ & SWE-Llama 13b & SWE-Llama 7b \\
\midrule
    2023        & 244 & 61  & 4.51 & 1.56 & 0.00 & 4.07 & 3.50 \\
    2022        & 395 & 117 & 4.05 & 0.85 & 3.42 & 2.80 & 2.46 \\
    2021        & 383 & 102 & 4.18 & 0.00 & 2.94 & 4.45 & 2.56 \\
    2020        & 427 & 109 & 5.15 & 0.71 & 0.00 & 3.96 & 3.43 \\
    2019        & 437 & 112 & 5.72 & 1.49 & 1.79 & 4.55 & 2.21 \\
    2018        & 165 & 37  & 5.45 & 0.00 & 0.00 & 3.57 & 2.94 \\
    $<$ 2018 & 89  & 36  & 4.49 & 0.00 & 2.78 & 3.37 & 1.09 \\
\bottomrule
\end{tabular}
\caption{
We present an extended temporal analysis in this table, showing the \% resolved for task instances across models in the ``Oracle" retrieval setting, separated by different cutoff dates. The \textit{Year} column refers to the subset of tasks that were created during the specified calendar year. In the \textit{Total} column, we list the number of tasks that fall within the given year. The \textit{$25$\%} column is the same information for the subset that GPT-4 was evaluated on. The remaining model-specific columns contain the \% resolved metric.
}
\label{appx:temporal-results-extended}
\end{table}

==> tables/bm25-results.tex <==
\begin{table}[ht]
\centering
\begin{minipage}[t]{0.48\textwidth}
    \centering
    \caption{
    Model resolve rates with BM25 retrieval, with different maximum context lengths.
    }
    \begin{tabular}{lccc}
        \toprule
         & \multicolumn{3}{c}{Max. Content} \\ \cmidrule(lr){2-4} 
        Model & $13$k & $27$k & $50$k \\    \cmidrule(lr){1-1}  \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}  
        Claude 2        & {\bf 1.96} & {\bf 1.87} & {\bf 1.22} \\
        SWE-Llama 7b    & 0.70 & 0.31 & 0.00 \\
        SWE-Llama 13b   & 0.70 & 0.48 & 0.00 \\
        \bottomrule
    \end{tabular}
    \label{table:bm25-results}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
    \centering
    \caption{
    BM25 recall with respect to  oracle files for different maximum context lengths.
    }
    \begin{tabular}{lccc}
        \toprule
        & \multicolumn{3}{c}{BM25 Recall} \\\cmidrule(lr){2-4}
        & $13$k & $27$k & $50$k \\  \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 
        Avg.& 29.58 & 44.41 & 51.06 \\
        All & 26.09 & 39.83 & 45.90 \\
        Any & 34.77 & 51.27 & 58.38 \\
        \bottomrule
    \end{tabular}
    \label{table:recall}
\end{minipage}
\end{table}

==> tables/main-results.tex <==
\begin{table}
\centering
\caption{
We compare models against each other using the BM25 retriever as described in Section~\ref{sec:experimental-setup}.
}
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{SWE-bench} & \multicolumn{2}{c}{SWE-bench Lite} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}  % Add rules under the multi-columns for clarity
Model & \% Resolved & \% Apply & \% Resolved & \% Apply \\
\midrule
Claude 3 Opus   & {\bf 3.79} & 46.56        & {\bf 4.33} & {\bf 51.67} \\
Claude 2        & 2.97       & 43.07        & 3.00       & 33.00       \\
ChatGPT-3.5     & 0.17       & 26.33        & 0.33       & 10.00       \\ 
GPT-4-turbo     & 1.31       & 26.90        & 2.67       & 29.67       \\
SWE-Llama 7b    & 0.70       & 51.74        & 1.33       & 38.00       \\
SWE-Llama 13b   & 0.70       & {\bf 53.62}  & 1.00       & 38.00       \\
\bottomrule
\end{tabular}
\label{table:main-results}
\end{table}


==> tables/model-context-comparision.tex <==
\begin{table}[ht]
    \centering
    \caption{
    We compare the different context lengths and proportion of the ``oracle" retrieval setting covered.
    Models with shorter context lengths are thus inherently disadvantaged.
    Note that descriptions of token-lengths is a relative non-standard measure (e.g. Llama-tokenized sequences are $42$\% longer on average than the equivalent sequence tokenized for GPT-4).
    }
    \begin{tabular}{lcccc}
    \toprule
                           & ChatGPT-3.5 & GPT-4 & Claude 2 & \swellama{} \\
    \midrule
    Max. Tokens  & \num{16385} & \num{32768} & \num{100000} & $\ge$\num{100000} \\
    \% of Instances   & 58.1\% & 84.1\% & 96.4\% & $\ge$94.8\%  \\
    \bottomrule
    \end{tabular}
    \label{tab:model-context-comparision}
\end{table}

==> tables/quantitative-analysis-gens.tex <==
\begin{table}[ht]
\centering
\caption{
Average edits of model generated patches in the ``oracle'' retrieval setting across successfully applied patches.
For the task instances specific to each model, we calculate the same statistics across the gold patches.
Avg Gold shows statistics macro-averaged over each models' respective gold patches.
All Gold shows statistics for all gold patches unconditioned on model performance.
}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
    Model & Total Lines & Added & Removed & Functions & Files \\ \cmidrule(lr){1-1} \cmidrule(lr){2-6}  
    Claude 2 & 19.6 & 4.2 & 1.9 & 1.1 & 1.0 \\
    \quad Gold & 44.1 & 12.0 & 5.8 & 2.1 & 1.2 \\
\midrule
    ChatGPT-3.5 & 30.1 & 3.8 & 2.7 & 1.6 & 1.0 \\
    \quad Gold & 39.6 & 9.5 & 6.1 & 1.9 & 1.2 \\
\midrule
    GPT-4 & 20.9 & 4.4 & 1.5 & 1.0 & 1.0 \\
    \quad Gold & 33.6 & 8.4 & 3.8 & 1.9 & 1.1 \\
\midrule
    SWE-Llama 13b & 17.6 & 1.6 & 1.2 & 1.2 & 1.1 \\
    \quad Gold & 37.8 & 10.0 & 4.4 & 1.9 & 1.1 \\
\midrule
    SWE-Llama 7b & 16.7 & 1.3 & 1.2 & 1.2 & 1.1 \\
    \quad Gold & 40.2 & 11.3 & 4.9 & 1.9 & 1.1 \\
\midrule
    Avg Gold & 39.1 & 10.2 &  5.0 & 1.9 & 1.1 \\
    All Gold & 74.5 & 22.3 & 10.5 & 3.0 & 1.7 \\
\bottomrule
\end{tabular}
}
\label{table:quantitative-analysis-gens}
\end{table}

==> tables/temporal-results.tex <==
\begin{table}[ht]
\centering
\caption{
We compare performance on task instances from before and after 2023 in the ``Oracle" retrieval setting.
Most models show little difference in performance. $^*$Due to budget constraints, GPT-4 is evaluated on a $25\%$ random subset of \benchmark{} tasks, which may impact performance.
}
\begin{tabular}{lccccc}
\toprule
    & Claude 2   & ChatGPT-3.5 & GPT-4$^*$  & SWE-Llama 7b & SWE-Llama 13b \\
\midrule
    Before 2023 & {\bf 4.87} & 0.49        & {\bf 1.96} & 2.95         & {\bf 3.98} \\
    After 2023   & 4.23       & {\bf 0.77}  & 0.0        & {\bf 3.46}   & {3.85} \\
\bottomrule
\end{tabular}
\label{table:temporal-results}
\end{table}

==> tables/two-turn-general-improvement.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of One-Turn vs. Two-Turn Performance}
\label{tab:two-turn-comparison}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \multicolumn{2}{c}{\textbf{Correctness}} & \multicolumn{2}{c}{\textbf{Passed Tests Share}} & \textbf{Improvement} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-6}
 & One-Turn & Two-Turn & One-Turn & Two-Turn & Correctness ($\Delta$) \\
\midrule
Claude 3.7 Sonnet & 0.340 & 0.640 & 0.531 & 0.716 & \textcolor{ForestGreen}{+0.300} \\
Claude 3.5 Sonnet V2 & 0.320 & 0.560 & 0.470 & 0.661 & \textcolor{ForestGreen}{+0.240} \\
Gemini 2.5 Pro (03-25 Preview) & 0.270 & 0.400 & 0.367 & 0.414 & \textcolor{ForestGreen}{+0.130} \\
DeepSeek R1 & 0.240 & 0.430 & 0.349 & 0.517 & \textcolor{ForestGreen}{+0.190} \\
GPT-4.1 (2025-04-14) & 0.180 & 0.480 & 0.264 & 0.559 & \textcolor{ForestGreen}{+0.300} \\
Mistral Large & 0.140 & 0.230 & 0.203 & 0.286 & \textcolor{ForestGreen}{+0.090} \\
LLaMA 4 Maverick 17B 128E Instruct FP8 & 0.080 & 0.180 & 0.130 & 0.237 & \textcolor{ForestGreen}{+0.100} \\
% Amazon Nova Pro & 0.010 & 0.070 & 0.045 & 0.133 & \textcolor{ForestGreen}{+0.060} \\
\bottomrule
\end{tabular}
}
\begin{flushleft}
\small
This table compares the performance of models in one-turn and two-turn settings:
% \begin{itemize}
\newline - \textbf{Correctness}: Binary success metric - 1 if solution passed all tests, 0 otherwise
\newline - \textbf{Passed Tests Share}: Share of tests passed for the task
\newline - \textbf{Improvement}: Increase in correctness from one- to two-turn approach (positive values imply improvement)
% \end{itemize}
\end{flushleft}
\end{table}

